Advancing vision-language models in front-end development via data synthesis

Modern front-end (FE) development, especially when leveraging the unique features of frameworks like React and Vue, presents distinctive challenges. These include managing modular architectures, ensuring synchronization between data and visual outputs for declarative rendering, and adapting reusable components to various scenarios. Such complexities make it particularly difficult for state-of-the-art large vision-language models (VLMs) to generate accurate and functional code directly from design images. To address these challenges, we propose a reflective agentic workflow that synthesizes high-quality image-text data to capture the diverse characteristics of FE development. This workflow automates the extraction of self-contained\footnote{A \textbf{self-contained} code snippet is one that encapsulates all necessary logic, styling, and dependencies, ensuring it functions independently without requiring external imports or context.} code snippets from real-world projects, renders the corresponding visual outputs, and generates detailed descriptions that link design elements to functional code. To further expand the scope and utility of the synthesis, we introduce three data synthesis strategies: Evolution-based synthesis, which enables scalable and diverse dataset expansion; Waterfall-Model-based synthesis, which generates logically coherent code derived from system requirements; and Additive Development synthesis, which iteratively increases the complexity of human-authored components. We build a large vision-language model, Flame, trained on the synthesized datasets and demonstrate its effectiveness in generating React code via the $\text{pass}@k$ metric. Our results suggest that a code VLM trained to interpret images before code generation may achieve better performance.

==> 00-outline.tex <==
\section{Outline [Not included in the main texts]}
FLAME: A Frontend Language Assistant with Multimodal Expertise

Contributions:\\
1. We build a pipeline for constructing front-end code snippet and rendered images\\
2. We proposed a variant of pass@k to evaluate the quality of FE code generated by the LVLM\\
3. We build a large vision and language model for generating FE codes\\

Problem statement:
\begin{enumerate}
    \item FE deveolopment, not simply on HTML, Very Hard Problem, 
    \item Method: multimodal data collection => construct and tuning the VLM => evaluate.
        \begin{itemize}
            \item Core part: how to build such data construction pipeline, with the agent workflow 
        \end{itemize}
    \item evaluation is still hard, propose a new way.
    \item Findings
        \begin{itemize}
            \item with Image or NOT
            \item vision encoder => perceiver
            \item pre-train data quantity: one vision vs 558k
            \item Parameters: 7B vs 33B optional
            \item data: variation useful?
                \begin{itemize}
                    * none vs 3 vs 10 vs 15
                    * instruction variations from
                \end{itemize}
        \end{itemize}
\end{enumerate}


==> 04-background.tex <==
\section{Background}
React stands as the cornerstone framework in the realm of modern web development, offering extensive capabilities that cater to a broad spectrum of front-end development scenarios. React utilizes a virtual DOM to enable efficient updates and rendering, making it highly suitable for dynamic applications that undergo frequent UI changes. Its component-based architecture not only fosters reusability but also streamlines scalability in projects. A typical React project is structured around several types of files, key among them are JavaScript (JS), JSX, and CSS (or pre-processor files like SCSS or LESS). JS files contain the logic of components, including handling state and responding to user inputs. JSX, an XML-like syntax extension for JavaScript, is used within JS files to describe the structure of the interface, allowing developers to write HTML-like code directly in JavaScript. This integration facilitates the development of dynamic user interfaces that update efficiently. Lastly, CSS or its pre-processed variants like SCSS or LESS are used to style these components, dictating the visual presentation of the UI elements defined in JSX.

By focusing our research on React, we aim to directly address the most common and diverse needs found in real-world web projects. We first proposed a dataset that combines React code snippets with corresponding design mockups. This dataset contains three parts: 1) a design mockup image, 2) a React code snippet, and 3) descriptive text that explains the functionality of the design. This dataset serves as the foundation for training a vision-language model that can generate code snippets from design mockups and descriptive text, in order to bridge the gap between visual design and code by generating accurate initial code drafts from design mockups, significantly enhancing developer productivity and ensuring greater fidelity to the design's original vision.

% \subsection{React}

% React is a JavaScript library for building user interfaces, primarily through the creation of components that manage their own state and render UI. A typical React project is structured around several types of files, key among them are JavaScript (JS), JSX, and CSS (or pre-processor files like SCSS or LESS). JS files contain the logic of components, including handling state and responding to user inputs. JSX, an XML-like syntax extension for JavaScript, is used within JS files to describe the structure of the interface, allowing developers to write HTML-like code directly in JavaScript. This integration facilitates the development of dynamic user interfaces that update efficiently. Lastly, CSS or its pre-processed variants like SCSS or LESS are used to style these components, dictating the visual presentation of the UI elements defined in JSX.

% \subsection{Vue}

% Vue is a progressive JavaScript framework used for building UIs and single-page applications. Vue projects are typically organized into single-file components (SFCs), which encapsulate the logic, layout, and style of components in a single file. These files commonly contain three types of code blocks: <template>, <script>, and <style>. The <template> block uses HTML-based syntax to define the layout of the component, the <script> block contains the JavaScript code responsible for the logic of the component, such as data handling and user interactions, and the <style> block includes the CSS that applies styles directly to this component. This structure promotes a modular and maintainable approach to development, as each component contains all aspects of its behavior and appearance in one place, making Vue highly adaptable and easy to integrate with other libraries or existing projects.

==> 0501-react.tex <==
% \subsection{React as the Target Framework}
% By centering our on React, our dataset aligns with common industry practices, ensuring relevance to real-world front-end development.

